ISA-bEL: Intelligent Search Algorithm based on Entity Linking

Nowadays, the way in which the people interact with computers has changed. Text- or voice-based interfaces are being widely applied in different industries. Among the most used ways of processing the user input are those based on intents or retrieval algorithms. In these solutions, important information of the user could be lost in the process. For the proposed natural language processing pipeline the entities are going to take a principal role, under the assumption that entities are where the purpose of the user resides. Entities fed with context will be projected to a specific domain supported by a knowledge graph, resulting in what has been named as linked entities. These linked entities serve then as a key for searching a top level aggregation concept within our knowledge graph.

==> citas.tex <==
@article{Miller2019,
   abstract = {There has been a recent resurgence in the area of explainable artificial intelligence as researchers and practitioners seek to provide more transparency to their algorithms. Much of this research is focused on explicitly explaining decisions or actions to a human observer, and it should not be controversial to say that looking at how humans explain to each other can serve as a useful starting point for explanation in artificial intelligence. However, it is fair to say that most work in explainable artificial intelligence uses only the researchers' intuition of what constitutes a ‘good’ explanation. There exist vast and valuable bodies of research in philosophy, psychology, and cognitive science of how people define, generate, select, evaluate, and present explanations, which argues that people employ certain cognitive biases and social expectations to the explanation process. This paper argues that the field of explainable artificial intelligence can build on this existing research, and reviews relevant papers from philosophy, cognitive psychology/science, and social psychology, which study these topics. It draws out some important findings, and discusses ways that these can be infused with work on explainable artificial intelligence.},
   author = {Tim Miller},
   doi = {https://doi.org/10.1016/j.artint.2018.07.007},
   issn = {0004-3702},
   journal = {Artificial Intelligence},
   keywords = {Explainability,Explainable AI,Explanation,Interpretability,Transparency},
   pages = {1-38},
   title = {Explanation in artificial intelligence: Insights from the social sciences},
   volume = {267},
   url = {https://www.sciencedirect.com/science/article/pii/S0004370218305988},
   year = {2019},
}

@ARTICLE{Galassi20214291,
author={Galassi, A. and Lippi, M. and Torroni, P.},
title={Attention in Natural Language Processing},
journal={IEEE Transactions on Neural Networks and Learning Systems},
year={2021},
volume={32},
number={10},
pages={4291-4308},
doi={10.1109/TNNLS.2020.3019893},
note={cited By 25},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85117224349&doi=10.1109%2fTNNLS.2020.3019893&partnerID=40&md5=677e4d61c8b510432fd342ca56a38541},
affiliation={Department of Computer Science and Engineering (DISI), University of Bologna, Bologna, 40126, Italy; Department of Sciences and Methods for Engineering (DISMI), University of Modena and Reggio Emilia, Modena, 41121, Italy},
abstract={Attention is an increasingly popular mechanism used in a wide range of neural architectures. The mechanism itself has been realized in a variety of formats. However, because of the fast-paced advances in this domain, a systematic overview of attention is still missing. In this article, we define a unified model for attention architectures in natural language processing, with a focus on those designed to work with vector representations of the textual data. We propose a taxonomy of attention models according to four dimensions: the representation of the input, the compatibility function, the distribution function, and the multiplicity of the input and/or output. We present the examples of how prior information can be exploited in attention models and discuss ongoing research efforts and open challenges in the area, providing the first extensive categorization of the vast body of literature in this exciting domain. © 2012 IEEE.},
author_keywords={Natural language processing (NLP);  neural attention;  neural networks;  review;  survey},
document_type={Article},
source={Scopus},
}
@incollection{abney1991parsing,
  title={Parsing by chunks},
  author={Abney, Steven P},
  booktitle={Principle-based parsing},
  pages={257--278},
  year={1991},
  publisher={Springer}
}
@inproceedings{chen2014fast,
  title={A fast and accurate dependency parser using neural networks},
  author={Chen, Danqi and Manning, Christopher D},
  booktitle={Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP)},
  pages={740--750},
  year={2014}
}
@ARTICLE{NIPS2017_3f5ee243,
 author = {Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, \L ukasz and Polosukhin, Illia},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Attention is All you Need},
 url = {https://proceedings.neurips.cc/paper/2017/file/3f5ee243547dee91fbd053c1c4a845aa-Paper.pdf},
 volume = {30},
 year = {2017}
}

@article{nadeau2007survey,
  title={A survey of named entity recognition and classification},
  author={Nadeau, David and Sekine, Satoshi},
  journal={Lingvisticae Investigationes},
  volume={30},
  number={1},
  pages={3--26},
  year={2007},
  publisher={John Benjamins}
}

@book{10.5555/3110856,
author = {Goldberg, Yoav and Hirst, Graeme},
title = {Neural Network Methods in Natural Language Processing},
year = {2017},
isbn = {1627052984},
publisher = {Morgan \& Claypool Publishers},
abstract = {Neural networks are a family of powerful machine learning models. This book focuses on the application of neural network models to natural language data. The first half of the book (Parts I and II) covers the basics of supervised machine learning and feed-forward neural networks, the basics of working with machine learning over language data, and the use of vector-based rather than symbolic representations for words. It also covers the computation-graph abstraction, which allows to easily define and train arbitrary neural networks, and is the basis behind the design of contemporary neural network software libraries. The second part of the book (Parts III and IV) introduces more specialized neural network architectures, including 1D convolutional neural networks, recurrent neural networks, conditioned-generation models, and attention-based models. These architectures and techniques are the driving force behind state-of-the-art algorithms for machine translation, syntactic parsing, and many other applications. Finally, we also discuss tree-shaped networks, structured prediction, and the prospects of multi-task learning.}
}

@article{tarwani2017survey,
  title={Survey on recurrent neural network in natural language processing},
  author={Tarwani, Kanchan M and Edem, Swathi},
  journal={Int. J. Eng. Trends Technol},
  volume={48},
  pages={301--304},
  year={2017}
}

@article{DBLP:journals/corr/abs-1909-09586,
  author    = {Ralf C. Staudemeyer and
               Eric Rothstein Morris},
  title     = {Understanding {LSTM} - a tutorial into Long Short-Term Memory Recurrent
               Neural Networks},
  journal   = {CoRR},
  volume    = {abs/1909.09586},
  year      = {2019},
  url       = {http://arxiv.org/abs/1909.09586},
  eprinttype = {arXiv},
  eprint    = {1909.09586},
  timestamp = {Tue, 24 Sep 2019 11:33:51 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1909-09586.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@ARTICLE{MusaAliyu2018157,
author={Musa Aliyu, F. and Ojo, A.},
title={Towards building a knowledge graph with open data – a roadmap},
journal={Lecture Notes of the Institute for Computer Sciences, Social-Informatics and Telecommunications Engineering, LNICST},
year={2018},
volume={250},
pages={157-162},
doi={10.1007/978-3-319-98827-6_13},
note={cited By 1},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85052830661&doi=10.1007%2f978-3-319-98827-6_13&partnerID=40&md5=9f314ffdeeab53f27006d8c39358af5c},
affiliation={Federal University Birnin Kebbi, Birnin Kebbi, Kebbi, Nigeria; Insight Centre for Data Analytics, National University of Ireland, Galway (NUIG), Galway, Ireland},
abstract={With the increasing interest in knowledge graph over the years, several approaches have been proposed for building knowledge graphs. Most of the recent approaches involve using semi-structured sources such as Wikipedia or information crawled from the web using a combination of extraction methods and Natural Language Processing (NLP) techniques. In most cases, these approaches tend to make a compromise between accuracy and completeness. In our ongoing work, we examine a technique for building a knowledge graph over the increasing volume of open data published on the web. The rationale for this is two-fold. First, we intend to provide a foundation for making existing open datasets searchable through keywords similar to how information is sought on the web. The second reason is to generate logically consistent facts from usually inaccurate and inconsistent open datasets. Our approach to knowledge graph development will compute the confidence score of every relationship elicited from underpinning open data in the knowledge graph. Our method will also provide a scheme for extending coverage of a knowledge graph by predicting new relationships that are not in the knowledge graph. In our opinion, our work has major implications for truly opening up access to the hitherto untapped value in open datasets not directly accessible on the World Wide Web today. © 2018, ICST Institute for Computer Sciences, Social Informatics and Telecommunications Engineering.},
author_keywords={Knowledge graph;  Open data},
document_type={Conference Paper},
source={Scopus},
}
@CONFERENCE{Ehrlinger2016,
author={Ehrlinger, L. and Wöß, W.},
title={Towards a definition of knowledge graphs},
booktitle={Towards a definition of knowledge graphs},
journal={CEUR Workshop Proceedings},
year={2016},
volume={1695},
note={cited By 19},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84992411277&partnerID=40&md5=b279d3579a1465608adf7586b0037de8},
affiliation={Institute for Application Oriented Knowledge Processing, Johannes Kepler University, Linz, Austria},
abstract={Recently, the term knowledge graph has been used frequently in research and business, usually in close association with Semantic Web technologies, linked data, large-scale data analytics and cloud computing. Its popularity is clearly influenced by the introduction of Google's Knowledge Graph in 2012, and since then the term has been widely used without a definition. A large variety of interpretations has hampered the evolution of a common understanding of knowledge graphs. Numerous research papers refer to Google's Knowledge Graph, although no official documentation about the used methods exists. The prerequisite for widespread academic and commercial adoption of a concept or technology is a common understanding, based ideally on a definition that is free from ambiguity. We tackle this issue by discussing and defining the term knowledge graph, considering its history and diversity in interpretations and use. Our goal is to propose a definition of knowledge graphs that serves as basis for discussions on this topic and contributes to a common vision. © 2016 Copyright held by the author/owner(s).s).},
author_keywords={Knowledge bases;  Knowledge graphs;  Knowledge representation;  Ontologies;  Semantic web},
document_type={Conference Paper},
source={Scopus},
}
@CONFERENCE{Suchanek2007697,
author={Suchanek, F.M. and Kasneci, G. and Weikum, G.},
title={Yago: A core of semantic knowledge},
booktitle={Towards a definition of knowledge graphs},
journal={16th International World Wide Web Conference, WWW2007},
year={2007},
pages={697-706},
doi={10.1145/1242572.1242667},
note={cited By 2260},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-35148867982&doi=10.1145%2f1242572.1242667&partnerID=40&md5=3b00d0d191fa288c389d6ec7e80b9474},
affiliation={Max-Planck-Institute for Computer Science, Saarbrücken, Germany},
abstract={We present YAGO, a light-weight and extensible ontology with high coverage and quality. YAGO builds on entities and relations and currently contains more than 1 million entities and 5 million facts. This includes the Is-A hierarchy as well as non-taxonomic relations between entities (such as HASONEPRIZE). The facts have been automatically extracted from Wikipedia and unified with WordNet, using a carefully designed combination of rule-based and heuristic methods described in this paper. The resulting knowledge base is a major step beyond WordNet: in quality by adding knowledge about individuals like persons, organizations, products, etc. with their semantic relationships - and in quantity by increasing the number of facts by more than an order of magnitude. Our empirical evaluation of fact correctness shows an accuracy of about 95%. YAGO is based on a logically clean model, which is decidable, extensible, and compatible with RDFS. Finally, we show how YAGO can be further extended by state-of-the-art information extraction techniques.},
author_keywords={Wikipedia;  WordNet},
document_type={Conference Paper},
source={Scopus},
}
@ARTICLE{Auer2007722,
author={Auer, S. and Bizer, C. and Kobilarov, G. and Lehmann, J. and Cyganiak, R. and Ives, Z.},
title={DBpedia: A nucleus for a Web of open data},
journal={Lecture Notes in Computer Science (including subseries Lecture Notes in Artificial Intelligence and Lecture Notes in Bioinformatics)},
year={2007},
volume={4825 LNCS},
pages={722-735},
doi={10.1007/978-3-540-76298-0_52},
note={cited By 2306},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-49949092526&doi=10.1007%2f978-3-540-76298-0_52&partnerID=40&md5=c8e7c42b844cebdb028c91f30065b849},
affiliation={Universität Leipzig, Department of Computer Science, Johannisgasse 26, D-04103 Leipzig, Germany; Freie Universität Berlin, Web-based Systems Group, Garystr. 21, D-14195 Berlin, Germany; University of Pennsylvania, Department of Computer and Information Science, Philadelphia, PA 19104, United States},
abstract={DBpedia is a community effort to extract structured information from Wikipedia and to make this information available on the Web. DBpedia allows you to ask sophisticated queries against datasets derived from Wikipedia and to link other datasets on the Web to Wikipedia data. We describe the extraction of the DBpedia datasets, and how the resulting information is published on the Web for human- and machine-consumption. We describe some emerging applications from the DBpedia community and show how website authors can facilitate DBpedia content within their sites. Finally, we present the current status of interlinking DBpedia with other open datasets on the Web and outline how DBpedia could serve as a nucleus for an emerging Web of open data. © 2008 Springer-Verlag Berlin Heidelberg.},
document_type={Conference Paper},
source={Scopus},
}
@ARTICLE{Vrande201478,
author={Vrandečić, D. and Krötzsch, M.},
title={Wikidata: A free collaborative knowledgebase},
journal={Communications of the ACM},
year={2014},
volume={57},
number={10},
pages={78-85},
doi={10.1145/2629489},
note={cited By 1092},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-84905830193&doi=10.1145%2f2629489&partnerID=40&md5=b2a7c5ba36d49753eaf49270a33e6c13},
affiliation={Google, San Francisco, CA, United States; Wikimedia Deutschland, Berlin, CT, United States; Technische Universität Dresden, Dresden, Germany},
abstract={Wikidata allows every user to extend and edit the stored information, even without creating an account. A form based interface makes editing easy. Wikidata's goal is to allow data to be used both in Wikipedia and in external applications. Data is exported through Web services in several formats, including JavaScript Object Notation, or JSON, and Resource Description Framework, or RDF. Data is published under legal terms that allow the widest possible reuse. The value of Wikipedia's data has long been obvious, with many efforts to use it. The Wikidata approach is to crowdsource data acquisition, allowing a global community to edit the data. This extends the traditional wiki approach of allowing users to edit a website. In March 2013, Wikimedia introduced Lua as a scripting language for automatically creating and enriching parts of articles. Lua scripts can access Wikidata, allowing Wikipedia editors to retrieve, process, and display data. Many other features were introduced in 2013, and development is planned to continue for the foreseeable future.},
document_type={Article},
source={Scopus},
}

@book{vasiliev2020natural,
  title={Natural Language Processing with Python and SpaCy: A Practical Introduction},
  author={Vasiliev, Yuli},
  year={2020},
  publisher={No Starch Press}
}
@inproceedings{webster1992tokenization,
  title={Tokenization as the initial phase in NLP},
  author={Webster, Jonathan J and Kit, Chunyu},
  booktitle={COLING 1992 Volume 4: The 14th International Conference on Computational Linguistics},
  year={1992}
}
@Inbook{Grefenstette1999,
author={Grefenstette, Gregory and van Halteren, Hans},
title="Tokenization",
bookTitle="Syntactic Wordclass Tagging",
year="1999",
publisher="Springer Netherlands",
address="Dordrecht",
pages="117--133",
abstract="The linguistic annotation of naturally occurring text can be seen as a progression of transformations of the original text, with each step abstracting away surface differences. Tokenization is one of the earliest steps in this transformation during natural language processing.",
isbn="978-94-015-9273-4",
doi="10.1007/978-94-015-9273-4_9",
url="https://doi.org/10.1007/978-94-015-9273-4_9"
}



@CONFERENCE{Chen20171870,
author={Chen, D. and Fisch, A. and Weston, J. and Bordes, A.},
title={Reading Wikipedia to answer open-domain questions},
booktitle={Reading Wikipedia to answer open-domain questions},
journal={ACL 2017 - 55th Annual Meeting of the Association for Computational Linguistics, Proceedings of the Conference (Long Papers)},
year={2017},
volume={1},
pages={1870-1879},
doi={10.18653/v1/P17-1171},
note={cited By 424},
url={https://www.scopus.com/inward/record.uri?eid=2-s2.0-85036663355&doi=10.18653%2fv1%2fP17-1171&partnerID=40&md5=87de418dc60c0bacd14f557392749189},
affiliation={Computer Science Stanford University, Stanford, CA  94305, United States; Facebook, AI Research, 770 Broadway, New York, NY  10003, United States},
abstract={This paper proposes to tackle open-domain question answering using Wikipedia as the unique knowledge source: the answer to any factoid question is a text span in a Wikipedia article. This task of machine reading at scale combines the challenges of document retrieval (finding the relevant articles) with that of machine comprehension of text (identifying the answer spans from those articles). Our approach combines a search component based on bigram hashing and TF-IDF matching with a multi-layer recurrent neural network model trained to detect answers in Wikipedia paragraphs. Our experiments on multiple existing QA datasets indicate that (1) both modules are highly competitive with respect to existing counterparts and (2) multitask learning using distant supervision on their combination is an effective complete system on this challenging task. © 2017 Association for Computational Linguistics.},
document_type={Conference Paper},
source={Scopus},
}
@article{harabagiu2003open,
  title={Open-domain textual question answering techniques},
  author={Harabagiu, Sanda M and Maiorano, Steven J and Pa{\c{s}}ca, Marius A},
  journal={Natural Language Engineering},
  volume={9},
  number={3},
  pages={231--267},
  year={2003},
  publisher={Cambridge University Press}
}

@article{khattab2021relevance,
  title={Relevance-guided supervision for openqa with colbert},
  author={Khattab, Omar and Potts, Christopher and Zaharia, Matei},
  journal={Transactions of the Association for Computational Linguistics},
  volume={9},
  pages={929--944},
  year={2021},
  publisher={MIT Press}
}
@article{karpukhin2020dense,
  title={Dense passage retrieval for open-domain question answering},
  author={Karpukhin, Vladimir and O{\u{g}}uz, Barlas and Min, Sewon and Lewis, Patrick and Wu, Ledell and Edunov, Sergey and Chen, Danqi and Yih, Wen-tau},
  journal={arXiv preprint arXiv:2004.04906},
  year={2020}
}
@inproceedings{nishida2018retrieve,
  title={Retrieve-and-read: Multi-task learning of information retrieval and reading comprehension},
  author={Nishida, Kyosuke and Saito, Itsumi and Otsuka, Atsushi and Asano, Hisako and Tomita, Junji},
  booktitle={Proceedings of the 27th ACM international conference on information and knowledge management},
  pages={647--656},
  year={2018}
}
@article{yang2019end,
  title={End-to-end open-domain question answering with bertserini},
  author={Yang, Wei and Xie, Yuqing and Lin, Aileen and Li, Xingyu and Tan, Luchen and Xiong, Kun and Li, Ming and Lin, Jimmy},
  journal={arXiv preprint arXiv:1902.01718},
  year={2019}
}

@article{rajpurkar2016squad,
  title={Squad: 100,000+ questions for machine comprehension of text},
  author={Rajpurkar, Pranav and Zhang, Jian and Lopyrev, Konstantin and Liang, Percy},
  journal={arXiv preprint arXiv:1606.05250},
  year={2016}
}
@article{hermann2015teaching,
  title={Teaching machines to read and comprehend},
  author={Hermann, Karl Moritz and Kocisky, Tomas and Grefenstette, Edward and Espeholt, Lasse and Kay, Will and Suleyman, Mustafa and Blunsom, Phil},
  journal={Advances in neural information processing systems},
  volume={28},
  year={2015}
}
@book{woods1997conceptual,
  title={Conceptual indexing: A better way to organize knowledge},
  author={Woods, William A},
  year={1997},
  publisher={Sun Microsystems, Inc.}
}
@article{molla2007question,
  title={Question answering in restricted domains: An overview},
  author={Moll{\'a}, Diego and Vicedo, Jos{\'e} Luis},
  journal={Computational Linguistics},
  volume={33},
  number={1},
  pages={41--61},
  year={2007},
  publisher={MIT Press One Rogers Street, Cambridge, MA 02142-1209, USA journals-info~…}
}
@inproceedings{green1961baseball,
  title={Baseball: an automatic question-answerer},
  author={Green Jr, Bert F and Wolf, Alice K and Chomsky, Carol and Laughery, Kenneth},
  booktitle={Papers presented at the May 9-11, 1961, western joint IRE-AIEE-ACM computer conference},
  pages={219--224},
  year={1961}
}
@article{qi2019answering,
  title={Answering complex open-domain questions through iterative query generation},
  author={Qi, Peng and Lin, Xiaowen and Mehr, Leo and Wang, Zijian and Manning, Christopher D},
  journal={arXiv preprint arXiv:1910.07000},
  year={2019}
}
@article{zhu2021retrieving,
  title={Retrieving and reading: A comprehensive survey on open-domain question answering},
  author={Zhu, Fengbin and Lei, Wenqiang and Wang, Chao and Zheng, Jianming and Poria, Soujanya and Chua, Tat-Seng},
  journal={arXiv preprint arXiv:2101.00774},
  year={2021}
}
@article{nakano2021webgpt,
  title={WebGPT: Browser-assisted question-answering with human feedback},
  author={Nakano, Reiichiro and Hilton, Jacob and Balaji, Suchir and Wu, Jeff and Ouyang, Long and Kim, Christina and Hesse, Christopher and Jain, Shantanu and Kosaraju, Vineet and Saunders, William and others},
  journal={arXiv preprint arXiv:2112.09332},
  year={2021}
}
@article{seo2019real,
  title={Real-time open-domain question answering with dense-sparse phrase index},
  author={Seo, Minjoon and Lee, Jinhyuk and Kwiatkowski, Tom and Parikh, Ankur P and Farhadi, Ali and Hajishirzi, Hannaneh},
  journal={arXiv preprint arXiv:1906.05807},
  year={2019}
}
@inproceedings{wang2018r,
  title={R 3: Reinforced ranker-reader for open-domain question answering},
  author={Wang, Shuohang and Yu, Mo and Guo, Xiaoxiao and Wang, Zhiguo and Klinger, Tim and Zhang, Wei and Chang, Shiyu and Tesauro, Gerry and Zhou, Bowen and Jiang, Jing},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}
@article{lewis2019bart,
  title={Bart: Denoising sequence-to-sequence pre-training for natural language generation, translation, and comprehension},
  author={Lewis, Mike and Liu, Yinhan and Goyal, Naman and Ghazvininejad, Marjan and Mohamed, Abdelrahman and Levy, Omer and Stoyanov, Ves and Zettlemoyer, Luke},
  journal={arXiv preprint arXiv:1910.13461},
  year={2019}
}
@article{raffel2019exploring,
  title={Exploring the limits of transfer learning with a unified text-to-text transformer},
  author={Raffel, Colin and Shazeer, Noam and Roberts, Adam and Lee, Katherine and Narang, Sharan and Matena, Michael and Zhou, Yanqi and Li, Wei and Liu, Peter J},
  journal={arXiv preprint arXiv:1910.10683},
  year={2019}
}
@inproceedings{wolf2020transformers,
  title={Transformers: State-of-the-art natural language processing},
  author={Wolf, Thomas and Debut, Lysandre and Sanh, Victor and Chaumond, Julien and Delangue, Clement and Moi, Anthony and Cistac, Pierric and Rault, Tim and Louf, R{\'e}mi and Funtowicz, Morgan and others},
  booktitle={Proceedings of the 2020 conference on empirical methods in natural language processing: system demonstrations},
  pages={38--45},
  year={2020}
}
@article{pan2009survey,
  title={A survey on transfer learning},
  author={Pan, Sinno Jialin and Yang, Qiang},
  journal={IEEE Transactions on knowledge and data engineering},
  volume={22},
  number={10},
  pages={1345--1359},
  year={2009},
  publisher={IEEE}
}
@software{cheftransformer,
  author = {Mehrdad Farahani, Kartik Godawat et.al.},
  month = {8},
  title = {{Chef Transformer}},
  url = {https://github.com/github/linguist},
  version = {},
  year = {2021}
}
@inproceedings{bien2020recipenlg,
  title={RecipeNLG: A cooking recipes dataset for semi-structured text generation},
  author={Bie{\'n}, Micha{\l} and Gilski, Micha{\l} and Maciejewska, Martyna and Taisner, Wojciech and Wisniewski, Dawid and Lawrynowicz, Agnieszka},
  booktitle={Proceedings of the 13th International Conference on Natural Language Generation},
  pages={22--28},
  year={2020}
}
@article{li2020survey,
  title={A survey on deep learning for named entity recognition},
  author={Li, Jing and Sun, Aixin and Han, Jianglei and Li, Chenliang},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={34},
  number={1},
  pages={50--70},
  year={2020},
  publisher={IEEE}
}
@inproceedings{luo2015joint,
  title={Joint entity recognition and disambiguation},
  author={Luo, Gang and Huang, Xiaojiang and Lin, Chin-Yew and Nie, Zaiqing},
  booktitle={Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing},
  pages={879--888},
  year={2015}
}
@article{reimers2019sentence,
  title={Sentence-bert: Sentence embeddings using siamese bert-networks},
  author={Reimers, Nils and Gurevych, Iryna},
  journal={arXiv preprint arXiv:1908.10084},
  year={2019}
}
@article{zhu2018exploiting,
  title={Exploiting semantic similarity for named entity disambiguation in knowledge graphs},
  author={Zhu, Ganggao and Iglesias, Carlos A},
  journal={Expert Systems with Applications},
  volume={101},
  pages={8--24},
  year={2018},
  publisher={Elsevier}
}
@article{arrieta2020explainable,
  title={Explainable Artificial Intelligence (XAI): Concepts, taxonomies, opportunities and challenges toward responsible AI},
  author={Arrieta, Alejandro Barredo and D{\'\i}az-Rodr{\'\i}guez, Natalia and Del Ser, Javier and Bennetot, Adrien and Tabik, Siham and Barbado, Alberto and Garc{\'\i}a, Salvador and Gil-L{\'o}pez, Sergio and Molina, Daniel and Benjamins, Richard and others},
  journal={Information fusion},
  volume={58},
  pages={82--115},
  year={2020},
  publisher={Elsevier}
}
@INPROCEEDINGS{9373074,
  author={Braşoveanu, Adrian M. P. and Andonie, Răzvan},
  booktitle={2020 24th International Conference Information Visualisation (IV)}, 
  title={Visualizing Transformers for NLP: A Brief Survey}, 
  year={2020},
  volume={},
  number={},
  pages={270-279},
  doi={10.1109/IV51561.2020.00051}}
  
@incollection{NIPS2017_7062,
title = {A Unified Approach to Interpreting Model Predictions},
author = {Lundberg, Scott M and Lee, Su-In},
booktitle = {Advances in Neural Information Processing Systems 30},
editor = {I. Guyon and U. V. Luxburg and S. Bengio and H. Wallach and R. Fergus and S. Vishwanathan and R. Garnett},
pages = {4765--4774},
year = {2017},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/7062-a-unified-approach-to-interpreting-model-predictions.pdf}
}
@inproceedings{lime,
  author    = {Marco Tulio Ribeiro and
               Sameer Singh and
               Carlos Guestrin},
  title     = {"Why Should {I} Trust You?": Explaining the Predictions of Any Classifier},
  booktitle = {Proceedings of the 22nd {ACM} {SIGKDD} International Conference on
               Knowledge Discovery and Data Mining, San Francisco, CA, USA, August
               13-17, 2016},
  pages     = {1135--1144},
  year      = {2016},
}
@Article{dlib09,
  author = {Davis E. King},
  title = {Dlib-ml: A Machine Learning Toolkit},
  journal = {Journal of Machine Learning Research},
  year = {2009},
  volume = {10},
  pages = {1755-1758},
}
@article{MALAMAS2021109,
title = {Embedding Rasa in edge Devices: Capabilities and Limitations},
journal = {Procedia Computer Science},
volume = {192},
pages = {109-118},
year = {2021},
note = {Knowledge-Based and Intelligent Information \& Engineering Systems: Proceedings of the 25th International Conference KES2021},
issn = {1877-0509},
doi = {https://doi.org/10.1016/j.procs.2021.08.012},
url = {https://www.sciencedirect.com/science/article/pii/S187705092101499X},
author = {Nikolaos Malamas and Andreas Symeonidis},
keywords = {Spoken Dialogue Systems, NLU, Rasa, Chatbots},
abstract = {Over the past few years, there has been a boost in the use of commercial virtual assistants. Obviously, these proprietary tools are well-performing, however the functionality they offer is limited, users are ”vendor-locked”, while possible user privacy issues rise. In this paper we argue that low-cost, open hardware solutions may also perform well, given the proper setup. Specifically, we perform an initial assessment of a low-cost virtual agent employing the Rasa framework integrated into a Raspberry Pi 4. We set up three different architectures, discuss their capabilities and limitations and evaluate the dialogue system against three axes: assistant comprehension, task success and assistant usability. Our experiments show that our low-cost virtual assistant performs in a satisfactory manner, even when a small-sized training dataset is used.}
}
@article{bocklisch2017rasa,
  title={Rasa: Open source language understanding and dialogue management},
  author={Bocklisch, Tom and Faulkner, Joey and Pawlowski, Nick and Nichol, Alan},
  journal={arXiv preprint arXiv:1712.05181},
  year={2017}
}
@InProceedings{overview_chatbot_2020,
author="Adamopoulou, Eleni
and Moussiades, Lefteris",
editor="Maglogiannis, Ilias
and Iliadis, Lazaros
and Pimenidis, Elias",
title="An Overview of Chatbot Technology",
booktitle="Artificial Intelligence Applications and Innovations",
year="2020",
publisher="Springer International Publishing",
address="Cham",
pages="373--383",
abstract="The use of chatbots evolved rapidly in numerous fields in recent years, including Marketing, Supporting Systems, Education, Health Care, Cultural Heritage, and Entertainment. In this paper, we first present a historical overview of the evolution of the international community's interest in chatbots. Next, we discuss the motivations that drive the use of chatbots, and we clarify chatbots' usefulness in a variety of areas. Moreover, we highlight the impact of social stereotypes on chatbots design. After clarifying necessary technological concepts, we move on to a chatbot classification based on various criteria, such as the area of knowledge they refer to, the need they serve and others. Furthermore, we present the general architecture of modern chatbots while also mentioning the main platforms for their creation. Our engagement with the subject so far, reassures us of the prospects of chatbots and encourages us to study them in greater extent and depth.",
isbn="978-3-030-49186-4"
}

@InProceedings{survey_design_2017,
author="Ramesh, Kiran
and Ravishankaran, Surya
and Joshi, Abhishek
and Chandrasekaran, K.",
editor="Kaushik, Saroj
and Gupta, Daya
and Kharb, Latika
and Chahal, Deepak",
title="A Survey of Design Techniques for Conversational Agents",
booktitle="Information, Communication and Computing Technology",
year="2017",
publisher="Springer Singapore",
address="Singapore",
pages="336--350",
abstract="A conversational agent also referred to as chatbot is a computer program which tries to generate human like responses during a conversation. Earlier chatbots employed much simpler retrieval based pattern matching design techniques. However, with time a number of new chatbots evolved with an aim to make it more human like and hence to pass the Turing test. Now, most of the chatbots employ generative knowledge based techniques. This paper will discuss about various chatbot design techniques, classification of chatbot and discussion on how the modern chatbots have evolved from simple pattern matching, retrieval based model to modern complex knowledge based models. A table of major conversational agents in chronological order along with their design techniques is also provided at the end of the paper.",
isbn="978-981-10-6544-6"
}
@article{yadav2020sentiment,
  title={Sentiment analysis using deep learning architectures: a review},
  author={Yadav, Ashima and Vishwakarma, Dinesh Kumar},
  journal={Artificial Intelligence Review},
  volume={53},
  number={6},
  pages={4335--4385},
  year={2020},
  publisher={Springer}
}
@INPROCEEDINGS{9076358,
  author={Rahul and Adhikari, Surabhi and Monika},
  booktitle={2020 Fourth International Conference on Computing Methodologies and Communication (ICCMC)}, 
  title={NLP based Machine Learning Approaches for Text Summarization}, 
  year={2020},
  volume={},
  number={},
  pages={535-538},
  doi={10.1109/ICCMC48092.2020.ICCMC-00099}}
  
  
@article{nlp_stateart,
author = {Khurana, Diksha and Koli, Aditya and Khatter, Kiran and Singh, Sukhdev},
year = {2017},
month = {08},
pages = {},
title = {Natural Language Processing: State of The Art, Current Trends and Challenges}
}

@article{usagesnlpdeeplearning,
  author    = {Daniel W. Otter and
               Julian R. Medina and
               Jugal K. Kalita},
  title     = {A Survey of the Usages of Deep Learning in Natural Language Processing},
  journal   = {CoRR},
  volume    = {abs/1807.10854},
  year      = {2018},
  url       = {http://arxiv.org/abs/1807.10854},
  eprinttype = {arXiv},
  eprint    = {1807.10854},
  timestamp = {Mon, 13 Aug 2018 16:46:19 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1807-10854.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{nlpareview,
author = {Joseph, Sethunya and Sedimo, Kutlwano and Kaniwa, Freeson and Hlomani, Hlomani and Letsholo, Keletso},
year = {2016},
month = {03},
pages = {207-210},
title = {Natural Language Processing: A Review},
volume = {6},
journal = {Natural Language Processing: A Review}
}

==> sections/section_results.tex <==
\section{experiments and results}



